A Note on Occur-Check

Most known results on avoiding the occur-check are based on the notion of "not subject to occur-check" (NSTO). It means that unification is performed only on such pairs of atoms for which the occur-check never succeeds in any run of a nondeterministic unification algorithm. Here we show that this requirement is too strong. We show how to weaken it, and present some related sufficient conditions under which the occur-check may be safely omitted. We show examples for which the proposed approach provides more general results than the approaches based on well-moded and nicely moded programs (this includes cases to which the latter approaches are inapplicable).

==> eptcsdata.tex <==
\providecommand{\firstpage}{54}
\providecommand{\publicationstatus}{A. Formisano, Y.A Liu, et al. (Eds.): International Conference on\\ Logic Programming (Technical Communications) 2021 (ICLP 2021)\\
EPTCS 345, 2021, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.345.17}{10.4204/EPTCS.345.17}}

